Improving Simulation Efficiency of MCMC for Inverse Modeling of Hydrologic Systems with a Kalman-Inspired Proposal Distribution

Bayesian analysis is widely used in science and engineering for real-time forecasting, decision making, and to help unravel the processes that explain the observed data. These data are some deterministic and/or stochastic transformations of the underlying parameters. A key task is then to summarize the posterior distribution of these parameters. When models become too difficult to analyze analytically, Monte Carlo methods can be used to approximate the target distribution. Of these, Markov chain Monte Carlo (MCMC) methods are particularly powerful. Such methods generate a random walk through the parameter space and, under strict conditions of reversibility and ergodicity, will successively visit solutions with frequency proportional to the underlying target density. This requires a proposal distribution that generates candidate solutions starting from an arbitrary initial state. The speed of the sampled chains converging to the target distribution deteriorates rapidly, however, with increasing parameter dimensionality. In this paper, we introduce a new proposal distribution that enhances significantly the efficiency of MCMC simulation for highly parameterized models. This proposal distribution exploits the cross-covariance of model parameters, measurements and model outputs, and generates candidate states much alike the analysis step in the Kalman filter. We embed the Kalman-inspired proposal distribution in the DREAM algorithm during burn-in, and present several numerical experiments with complex, high-dimensional or multi-modal target distributions. Results demonstrate that this new proposal distribution can greatly improve simulation efficiency of MCMC. Specifically, we observe a speed-up on the order of 10-30 times for groundwater models with more than one-hundred parameters.

==> trackchanges-0.7.0/README <==

TrackChanges
Multiple editors in LaTeX.
========================================================================

INTRODUCTION:

  The TrackChanges package consists of two parts:
  1.  A LaTex style file: 
        trackchanges.sty
  2.  A GUI, written in python:
         trackchanges.py

  The style file may be used without the GUI.  The GUI is to be used to
  facilitate accepting, rejecting, or modifying the edits made using the
  commands defined in the style file.

  This packages also includes a command line utility: acceptchanges.py.
  This utility will only work in posix environments.

  Help files are available as part of this package:
    ./documentation/web/help.html

  Documentation is also  available at the TrackChanges website.

  To get the latest version of this sofware go to:
    http://trackchanges.sourceforge.net

========================================================================

LaTeX STYLEFILE:

  INSTALLATION:
    Copy the style file to the directory with your LaTeX document.
    The style file can be found at: ./LatexPackage/trackchanges.sty

  USAGE:
    Add the following line to you latex document:
      \usepackage{trackchanges}

    Add the names of the editors in the preamble [OPTIONAL]:
      \addeditor{editor}

    Now you have access to all of the TrackChanges commands:
      \add[editor]{added text}
      \remove[editor]{removed text}
      \change[editor]{removed text}{added text}
      \note[editor]{note text}
      \annote[editor]{text to annotate}{note text}

    See the documentation or website for display options.

========================================================================

TRACKCHANGES GUI

  This is a Beta version of the TrackChanges GUI. 
  That means: Beware! Bugs may lurk ahead.

  If you choose to use this software plese be careful to back up your 
  TeX files.  This software has not been thoroughly tested and may
  corrupt your TeX files.  (The style file is fine and can't mess any
  thing up but the GUI for accepting/rejecting/modifying might.)

  ----------------------------------------------------------------------
  
  WARNING:  
    This program has not be generalized to handle international
    characters.  Such characters may cause unexpected behavior.
  
  NOTE:
    So far the GUI has only been tested on Windows XP and Os X.
    While it should work on linux, it might not.
  
  WARNING (AGAIN):
    This is beta software. It has not been tested much.
    Things may be broken.
  
  
  
  ----------------------------------------------------------------------
  INSTALLATION:
    Once you have all the dependencies installed, 
    just run ./PythonPackage/trackchanges.py
    
      $> cd PythonPackage
      $> python trackchanges.py
  
  
  ----------------------------------------------------------------------
  DEPENDANCIES:
    To get the trackchanges GUI to run you will need several things:
     
    1. Python 2.6 or later
    2. PyQt 4.4.4 or later
  
  ----------------------------------------------------------------------
  WHERE TO GET DEPENDANCIES:
    Python 2.6  -- http://www.python.org/
    PyQt 4      -- http://www.riverbankcomputing.co.uk/
  
  


========================================================================

This file is part of TrackChanges
Copyright 2009 Novimir Antoniuk Pablant
               Felix Salfner

TrackChanges is free software: you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation, either version 2 of the License, or
(at your option) any later version.

TrackChanges is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with TrackChanges.  If not, see <http://www.gnu.org/licenses/>.

------------------------------------------------------------------------
